FinLlama: Financial Sentiment Classification for Algorithmic Trading Applications

There are multiple sources of financial news online which influence market movements and trader's decisions. This highlights the need for accurate sentiment analysis, in addition to having appropriate algorithmic trading techniques, to arrive at better informed trading decisions. Standard lexicon based sentiment approaches have demonstrated their power in aiding financial decisions. However, they are known to suffer from issues related to context sensitivity and word ordering. Large Language Models (LLMs) can also be used in this context, but they are not finance-specific and tend to require significant computational resources. To facilitate a finance specific LLM framework, we introduce a novel approach based on the Llama 2 7B foundational model, in order to benefit from its generative nature and comprehensive language manipulation. This is achieved by fine-tuning the Llama2 7B model on a small portion of supervised financial sentiment analysis data, so as to jointly handle the complexities of financial lexicon and context, and further equipping it with a neural network based decision mechanism. Such a generator-classifier scheme, referred to as FinLlama, is trained not only to classify the sentiment valence but also quantify its strength, thus offering traders a nuanced insight into financial news articles. Complementing this, the implementation of parameter-efficient fine-tuning through LoRA optimises trainable parameters, thus minimising computational and memory requirements, without sacrificing accuracy. Simulation results demonstrate the ability of the proposed FinLlama to provide a framework for enhanced portfolio management decisions and increased market returns. These results underpin the ability of FinLlama to construct high-return portfolios which exhibit enhanced resilience, even during volatile periods and unpredictable market events.

==> setup/macro.tex <==
%% Custom commands
%% ===============

%% logo command
%\newcommand{\logo}[1][\textwidth]{\resizebox{#1}{!}{\includegraphics{setup/logo}}}

%% Ian Goodfellow LaTeX commands for math.
%%%%% NEW MATH DEFINITIONS %%%%%

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
%\def\rm{{\textnormal{m}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Random vectors with arrow
\def\rvvepsilon{{\vec{\mathbf{\epsilon}}}}
\def\rvvtheta{{\vec{\mathbf{\theta}}}}
\def\rvva{{\vec{\mathbf{a}}}}
\def\rvvb{{\vec{\mathbf{b}}}}
\def\rvvc{{\vec{\mathbf{c}}}}
\def\rvvd{{\vec{\mathbf{d}}}}
\def\rvve{{\vec{\mathbf{e}}}}
\def\rvvf{{\vec{\mathbf{f}}}}
\def\rvvg{{\vec{\mathbf{g}}}}
\def\rvvh{{\vec{\mathbf{h}}}}
\def\rvvu{{\vec{\mathbf{i}}}}
\def\rvvj{{\vec{\mathbf{j}}}}
\def\rvvk{{\vec{\mathbf{k}}}}
\def\rvvl{{\vec{\mathbf{l}}}}
\def\rvvm{{\vec{\mathbf{m}}}}
\def\rvvn{{\vec{\mathbf{n}}}}
\def\rvvo{{\vec{\mathbf{o}}}}
\def\rvvp{{\vec{\mathbf{p}}}}
\def\rvvq{{\vec{\mathbf{q}}}}
\def\rvvr{{\vec{\mathbf{r}}}}
\def\rvvs{{\vec{\mathbf{s}}}}
\def\rvvt{{\vec{\mathbf{t}}}}
\def\rvvu{{\vec{\mathbf{u}}}}
\def\rvvv{{\vec{\mathbf{v}}}}
\def\rvvw{{\vec{\mathbf{w}}}}
\def\rvvx{{\vec{\mathbf{x}}}}
\def\rvvy{{\vec{\mathbf{y}}}}
\def\rvvz{{\vec{\mathbf{z}}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vlambda{{\bm{\lambda}}}
\def\vmu{{\bm{\mu}}}
\def\valpha{{\bm{\alpha}}}
\def\vbeta{{\bm{\beta}}}
\def\vgamma{{\bm{\gamma}}}
\def\vtheta{{\bm{\theta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vomega{{\bm{\omega}}}
\def\vpsi{{\bm{\psi}}}
\def\vphi{{\bm{\phi}}}
\def\vsigma{{\bm{\sigma}}}
\def\vSigma{{\bm{\Sigma}}}
\def\veta{{\bm{\eta}}}
\def\vrho{{\bm{\rho}}}
\def\vRho{{\bm{\Rho}}}
\def\vphi{{\bm{\phi}}}
\def\vPhi{{\bm{\Phi}}}
\def\vDelta{{\bm{\Delta}}}
\def\vdelta{{\bm{\delta}}}

% Vectors with arrow
\def\vvzero{{\vec{\bm{0}}}}
\def\vvone{{\vec{\bm{1}}}}
\def\vva{{\vec{\bm{a}}}}
\def\vvb{{\vec{\bm{b}}}}
\def\vvc{{\vec{\bm{c}}}}
\def\vvd{{\vec{\bm{d}}}}
\def\vve{{\vec{\bm{e}}}}
\def\vvf{{\vec{\bm{f}}}}
\def\vvg{{\vec{\bm{g}}}}
\def\vvh{{\vec{\bm{h}}}}
\def\vvi{{\vec{\bm{i}}}}
\def\vvj{{\vec{\bm{j}}}}
\def\vvk{{\vec{\bm{k}}}}
\def\vvl{{\vec{\bm{l}}}}
\def\vvm{{\vec{\bm{m}}}}
\def\vvn{{\vec{\bm{n}}}}
\def\vvo{{\vec{\bm{o}}}}
\def\vvp{{\vec{\bm{p}}}}
\def\vvq{{\vec{\bm{q}}}}
\def\vvr{{\vec{\bm{r}}}}
\def\vvs{{\vec{\bm{s}}}}
\def\vvt{{\vec{\bm{t}}}}
\def\vvu{{\vec{\bm{u}}}}
\def\vvv{{\vec{\bm{v}}}}
\def\vvw{{\vec{\bm{w}}}}
\def\vvx{{\vec{\bm{x}}}}
\def\vvy{{\vec{\bm{y}}}}
\def\vvz{{\vec{\bm{z}}}}
\def\vvlambda{{\vec{\bm{\lambda}}}}
\def\vvmu{{\vec{\bm{\mu}}}}
\def\vvalpha{{\vec{\bm{\alpha}}}}
\def\vvbeta{{\vec{\bm{\beta}}}}
\def\vvgamma{{\vec{\bm{\gamma}}}}
\def\vvtheta{{\vec{\bm{\theta}}}}
\def\vvepsilon{{\vec{\bm{\epsilon}}}}
\def\vvomega{{\vec{\bm{\omega}}}}
\def\vvpsi{{\vec{\bm{\psi}}}}
\def\vvphi{{\vec{\bm{\phi}}}}
\def\vvsigma{{\vec{\bm{\sigma}}}}
\def\vvSigma{{\vec{\bm{\Sigma}}}}
\def\vveta{{\vec{\bm{\eta}}}}
\def\vvrho{{\vec{\bm{\rho}}}}
\def\vvRho{{\vec{\bm{\Rho}}}}
\def\vvphi{{\vec{\bm{\phi}}}}
\def\vvPhi{{\vec{\bm{\Phi}}}}
\def\vvDelta{{\vec{\bm{\Delta}}}}
\def\vvdelta{{\vec{\bm{\delta}}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Matrix with arrow
\def\mvA{{\vec{\bm{A}}}}
\def\mvB{{\vec{\bm{B}}}}
\def\mvC{{\vec{\bm{C}}}}
\def\mvD{{\vec{\bm{D}}}}
\def\mvE{{\vec{\bm{E}}}}
\def\mvF{{\vec{\bm{F}}}}
\def\mvG{{\vec{\bm{G}}}}
\def\mvH{{\vec{\bm{H}}}}
\def\mvI{{\vec{\bm{I}}}}
\def\mvJ{{\vec{\bm{J}}}}
\def\mvK{{\vec{\bm{K}}}}
\def\mvL{{\vec{\bm{L}}}}
\def\mvM{{\vec{\bm{M}}}}
\def\mvN{{\vec{\bm{N}}}}
\def\mvO{{\vec{\bm{O}}}}
\def\mvP{{\vec{\bm{P}}}}
\def\mvQ{{\vec{\bm{Q}}}}
\def\mvR{{\vec{\bm{R}}}}
\def\mvS{{\vec{\bm{S}}}}
\def\mvT{{\vec{\bm{T}}}}
\def\mvU{{\vec{\bm{U}}}}
\def\mvV{{\vec{\bm{V}}}}
\def\mvW{{\vec{\bm{W}}}}
\def\mvX{{\vec{\bm{X}}}}
\def\mvY{{\vec{\bm{Y}}}}
\def\mvZ{{\vec{\bm{Z}}}}
\def\mvBeta{{\vec{\bm{\beta}}}}
\def\mvPhi{{\vec{\bm{\Phi}}}}
\def\mvLambda{{\vec{\bm{\Lambda}}}}
\def\mvSigma{{\vec{\bm{\Sigma}}}}

% Tensor
% Got this from here: http://tex.stackexchange.com/questions/77640/bold-italic-and-sans-serif-math-symbols
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}

% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Matrix elements
% NOTE: we changed these from lower case to upper case to avoid
% clashes between vectors and matrices with same letter name.
% For example, we don't want elements of the hidden layer vector
% h to have the same name as elements of the Hessian matrix H
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% Tensor elements
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data-generating distribution
\newcommand{\pdata}{p_{\text{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\text{data}}}
\def\empirical{\ptrain} % Accidental duplicate
\newcommand{\Ptrain}{\hat{P}_{\text{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\text{model}}}
\newcommand{\Pmodel}{P_{\text{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\text{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\text{encoder}}}
\newcommand{\pdecode}{p_{\text{decoder}}}
\newcommand{\precons}{p_{\text{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution, see first use in prob.tex

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma} % Note: main text often hardcodes \sigma still, also
% many equations would likely frame bust if expanded to say \mathrm{sigmoid}
\newcommand{\sigm}{\sigmoid} % Duplicate command, this one is deprecated
\newcommand{\softplus}{\zeta} % Note: some figures may not use this macro, but main text consistently does
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\corr}{\mathrm{corr}}
\newcommand{\skewness}{\mathrm{skew}}
\newcommand{\kurtosis}{\mathrm{kurt}}
% Put these here so we can keep same syntax throughout the book but also change
% it easily.
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
% No one really seems to use subscripts (l_2, L_2) on general math reference
% sites, though subscripts seem popular in machine learning.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

% NOTE: This one was not done with a macro originally, many uses need to converted
% to \parents rather than Pa if we want to change it.
\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

%% Fixed/scaling delimiter examples (see mathtools documentation)
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

%% Use the alternative epsilon per default and define the old one as \oldepsilon
\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\ensuremath\varepsilon}

%% Also set the alternate phi as default.
\let\oldphi\phi
\renewcommand{\phi}{\ensuremath{\varphi}}

%% Text over sign.
\newcommand{\textoversign}[2]{\overset{\mathclap{\strut\text{#2}}}#1}

%% Statistics symbols
\def\E{{\mathbb{E}}}

%% Distributions (from Dan Dervovic)
\newcommand{\quaddist}{\ensuremath\operatorname{UQuadratic}}
\newcommand{\udist}{\ensuremath\operatorname{Uniform}}
\newcommand{\bernoulli}{\ensuremath\operatorname{Bernoulli}}
\newcommand{\expodist}{\ensuremath\operatorname{Exponential}}

%% ABIDES Agent Functions (from Dan Dervovic)
\newcommand{\wakeup}{\ProgSty{wakeup\_at}}
\newcommand{\marketorder}{\ProgSty{place\_market\_order}}
\newcommand{\limitorder}{\ProgSty{place\_limit\_order}}
\newcommand{\validtime}{\ProgSty{is\_valid\_time}}
\newcommand{\simrunning}{\ProgSty{sim\_running}}
\newcommand{\marketopen}{\ProgSty{market\_open}}
\newcommand{\bestbid}{\ProgSty{get\_best\_bid}}
\newcommand{\bestask}{\ProgSty{get\_best\_ask}}
\newcommand{\cancelorders}{\ProgSty{cancel\_all\_orders}}
\newcommand{\transactedvolume}{\ProgSty{get\_transacted\_volume}}
\newcommand{\buyvolume}{\ProgSty{get\_buy\_volume}}
\newcommand{\sellvolume}{\ProgSty{get\_sell\_volume}}
\newcommand{\currenttime}{\ProgSty{current\_time}}
\newcommand{\inventory}{\ProgSty{inventory}}
